An Efficient Algorithm for Computing High-Quality Paths amid Polygonal Obstacles

We study a path-planning problem amid a set $\mathcal{O}$ of obstacles in $\mathbb{R}^2$, in which we wish to compute a short path between two points while also maintaining a high clearance from $\mathcal{O}$; the clearance of a point is its distance from a nearest obstacle in $\mathcal{O}$. Specifically, the problem asks for a path minimizing the reciprocal of the clearance integrated over the length of the path. We present the first polynomial-time approximation scheme for this problem. Let $n$ be the total number of obstacle vertices and let $\varepsilon \in (0,1]$. Our algorithm computes in time $O(\frac{n^2}{\varepsilon ^2} \log \frac{n}{\varepsilon})$ a path of total cost at most $(1+\varepsilon)$ times the cost of the optimal path.

==> overview.tex <==
\section{Algorithm overview}
\label{sec:overview}
Our algorithm for solving the approximate weighted shortest-paths problem
borrows ideas from the Wein algorithm.
Specifically, we construct the Voronoi diagram~$\calV$ and subdivide it into intervals of length $\cl(I)\eps/24n$ in a similar fashion as described in Section~\ref{sec:alg_back}. These, in turn, induces a graph~$\calG$.\footnote{We intentionally use~$\calG$ to denote our graph and not~$\calD$ as described in Section~\ref{sec:alg_back} to avoid confusion between the two.}
Our algorithm differs both with respect to 
the intervals used as vertices and 
the edges used.
Specifically~$\calG$ uses a subset of the vertices edges of~$\calD$.

We overview our algorithm in two stages.
We first describe how to use only a subset of the vertices of~$\calD$ 
(while using the same rule to connect edges as in the Wein algorithm).
We then show how to reduce the number of edges considered using tools for approximating Euclidean shortest paths.


\paragraph{Simple $(n, \frac{1}{\varepsilon})$-near-optimal weighted shortest paths}
Let $\gamma^*$ be the 
shortest path between~$s$ and~$t$ and let $d^* = L^*(\gamma^*)$ be its length.
We later show how to compute an upper bound on $d^*$ and how this bound can be used to obtain our approximation algorithm.

We start by noting a simple, yet helpful observation.
Let $\lambda$ be Voronoi arc, 
defined by two obstacle features $o_1, o_2$ and
assume that $o_1, o_2$ are the only obstacles.
For every point $x$ lying on $\lambda$, 
denote by $L^*(s,x)$ and $L^*(t,x)$ the cost of the shortest path connecting $s$ and $t$ to $x$, respectively.
If $L^*(s,x) +  L^*(x,t)> d^*$ 
when only taking $o_1$ and $o_2$ into account
then the optimal path between~$s$ and~$t$ cannot pass through $x$.
This is true because travel costs only increase when additional obstacles are added.
We refer to all points~$x$ lying on a Voronoi arc~$\lambda$ such that 
$L^*(s,x) +  L^*(x,t) \leq d^*$ as $(s,t)$-\emph{promising points}
and we denote by $\calV_{d^*}(s,t)$ all the $(s,t)$-promising points lying on~$\calV$. 
The vertices of~$\calG$ are simply all the vertices of~$\calD$ which are contained in $\calV_{d^*}(s,t)$. 

We will show the total length of $\calV_{d^*}(s,t)$, 
denoted by~$\Lambda_{d^*}(s,t)$ is bounded $O(n d^*)$.
Additionally, we will show how to compute a path whose length is~$d_{max}^* =O(nd^*)$.
Hence, if we use $d_{max}^*$ instead of $d^*$, the total length of the Voronoi diagram used will be $O(n^2 d^*)$.
This allows, following exactly the same analysis as for the Wein algorithm, to deduce that considering only $(s,t)$-\emph{promising points} algorithm runs in time 
$
O 	\left(
		\left(d^*\right)^2 \cdot
		\left(1 / \eps^2 \right) \cdot
		n^{13/2}\log n
	\right)
$
(assuming that finding all such intervals does not incur additional overhead),
and returns a path whose weighted length is at most~$\eps$ longer than the weighted length of the optimal path.

\paragraph{Sparse $(n, \frac{1}{\varepsilon})$-near-optimal weighted shortest paths}
To further reduce the running time of our algorithm, we show how to use only a linear number of edges in~$\calD$ (linear in~$N$).
This will allow to reduce the running time of our algorithm to
$
O 	\left(
		d^* \cdot
		\left(1 / \eps \right) \cdot
		n^{7/2}\log n
	\right)
$
while adding a multiplicative factor of $1+\eps$ to the length of the solution returned by our algorithm.

\paragraph{Missing details}
Our high-level overview requires the following:
\begin{itemize}
	\item 	Bounding $\Lambda_{d^*}(s,t)$. 
			Namely, the length of~$\calV_{d^*}(s,t)$.
	\item 	Bounding $d^*$,
			the length of the optimal path~$\gamma^*$.
	\item	Showing how to compute $(s,t)$-promising points.
	\item	Showing how to use only a linear number of edges.\oren{this should move to the prev paragraph}
\end{itemize} 


==> point_obs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Point obstacles}
\label{sec:point_obs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we propose an efficient algorithm  for solving the approximate weighted shortest-paths problem
for a point robot amidst \emph{point} obstacles.
Our algorithm borrows ideas from the Wein algorithm described in Section~\ref{sec:alg_back}.
Similar to the Wein algorithm we use a discrete set of samples.
These samples are defined by defining intervals over the edges of~$\calV$ and choosing one point in each interval.
We then perform a Dijkstra-like pass on a graph induced by these samples.
Our algorithm differs both with respect to 
the intervals used as vertices and 
the edges used.
We start by motivating our algorithm and continue with a high-level overview, we then present the necessary technical details.


\paragraph{Motivation}
Let $\gamma^*$ be the 
shortest path between~$s$ and~$t$ and let $d^* = L^*(\gamma^*)$ be its length.
We later show how to compute an upper bound on $d^*$ and how this bound can be used to obtain our approximation algorithm.

We start by noting a simple, yet helpful observation.
Let $\lambda$ be Voronoi arc, 
defined by two obstacle features $o_1, o_2$ and
assume that $o_1, o_2$ are the only obstacles.
For every point $x$ lying on $\lambda$, 
denote by $L^*(s,x)$ the cost of the shortest path connecting $s$ to $x$.
If $L^*(s,x)> d^*$ 
when only taking $o_1$ and $o_2$ into account
then the optimal path between~$s$ and~$t$ cannot pass through $x$.
This is true because travel costs only increase when additional obstacles are added.
We refer to all points~$x$ lying on a Voronoi arc~$\lambda$ such that 
$L^*(s,x) \leq d^*$ as \emph{promising points}.

Thus, we wish to limit the Dijkstra-like search to traverse promising points nodes only.
These nodes will not be explicitly constructed in advance but gradually computed during the search.
Limiting our search to promising points only will allow us to traverse a considerably smaller set of vertices than the Wein algorithm. 
Moreover, to reduce the number of edges we construct a spanner over the set of edges connecting these nodes.
Again, the spanner will be constructed in an on-line fashion.


\paragraph{High-level description}
Our algorithm computes the Voronoi diagram~$\calV$ of the point obstacles and triangulates each Voronoi cell by connecting every vertex to its site\oren{we may need to split each triangle with the perpendicular line as well. If so, update Fig.~1}.
It then adds~$s$ and~$t$ as additional vertices and splits 
the triangles containing them into three triangles each (See Fig.~\ref{fig:vor_subdivision}).
It then computes an $O(n)$ approximation of $d^*$.
Now, Dijkstra's algorithm is run by adding~$s$ to priority queue~$\calQ$.
The rest of the vertices and edges traversed by the Dijkstra's algorithm will be computed during the search.

Suppose a vertex~$u$ is extracted from~$\calQ$ and let $T$ be a triangle 
(in the triangulation of~$\calV$) that contains~$u$ on its boundary. 
If all the edges of~$T$ have already been sampled and a 
spanner within~$T$ has been computed, 
then the search updates the cost of the neighbors of~$u$ in~$T$.
Otherwise, for each (at most two) edge~$e$ of~$T$ 
on which the points have not been sampled, 
we would like to compute all promising nodes.
As we will see, it is sufficient to sample at most $O(\frac{n}{\eps})$ points on~$e$ such that the points are sampled at intervals of weighted length $O(\frac{\eps \OPT}{n})$.
We add all the points sampled to~$\calQ$ together with the edges of the $\theta$-graph computed over these points. This ensures that the number of edges added is small while allowing to maintain near-optimal path lengths.




%More specifically, once we find the first point~$v$ on an edge~$e$, 
%we need to sample points at distance at most $2\OPT$\oren{this constant may should be worked out, it could be slightly larger since we don't get the closest point to $u$... } in each direction along~$e$. 
%
%
%
%Ideally, this would be done by computing the point~$x$ on~$e$ such that $L^*(u,x)$ is minimal, and walking on~$e$ in both directions by sampling points 
%We would then like to define intervals such that 
%
%
%As this is non-trivial, we compute a point~$v$ on~$e$ 
%such that $L^*(u,v) \leq 2 d^*$
%
%
%the point~$x$ on~$e$ 
%such that $L^*(u,x)$ is minimal.
%As this is non-trivial, we compute a point~$v$ on~$e$ 
%such that 
%\begin{equation}
%	\label{eq:almost-closest}
%	L^*(u,v) \leq \alpha \cdot \min_{x \in e} L^*(u,x).
%\end{equation}
%We then go at most $\alpha \cdot d^*$ in each direction along~$e$ from~$v$ 
%and sample uniformly along the edge. 
%We add all the points sampled to~$\calQ$ together with edges computed using a spanner\oren{ELABORATE}.

As we will see in the analysis this will give an algorithm that runs in time
%\footnote{The notation $\tilde{O}(\cdot)$ hides poly-logarithmic factors.} 
$
O \left( \frac{n^2}{\varepsilon} \log \frac{n}{\eps} \right )
$ and returns a solution whose cost has a multiplicative factor of $1 + \eps$ the cost of the upper bound on the optimal path and an additive factor of $\eps$.
Thus, we run our algorithm in iterations, at each iteration using half the cost of the previous iteration as a bound on~$d^*$. 
As our initial bound on~$d^*$ is by a factor of $O(n)$, after $O(\log n)$ iterations we obtain a solution whose cost~$d$ is bounded by 
$$
	d \leq (1 + \eps) \cdot d^* + \eps.
$$

\paragraph{Technical details}
To complete the description of our algorithm we still need to provide the following:
(i)~how to compute an $O(n)$ approximation of $d^*$,
(ii)~how to compute the promising nodes of each edge and
(iii)~how to build a spanner within each triangle~$T$.
%\begin{itemize}
%	\item 	Computing  an $O(n)$ approximation of $d^*$.
%	\item	Approximating the closest point on an edge~$e$ of~$\calV$ from a point 
%			in the same Voronoi cell.
%	\item	How points are sampled along the edge of~$\calV$
%	\item	The spanner construction.
%\end{itemize} 
We then show that the aforementioned algorithm indeed solves the approximate weighted shortest-paths problem and discuss the complexity of our algorithm.


\begin{figure}[tb]
  \centering
   	\includegraphics[height =5.0 cm]{./Voronoi_subdivision.pdf}
	\caption{\sf 	\footnotesize
				Triangulation of the Voronoi diagram~$\calV$ 
				of the set of obstacles 
				(black crosses surrounded by brown circles).
				Original edges of~$\calV$ and edges added due 
				to the triangulation are depicted using solid and dashed 
				lines,respectively.}
  \label{fig:vor_subdivision}
\end{figure}



\subsection{Transformed plane}
Recall that Eq.~\ref{eq:length_point} describes the cost of the shortest path between two points $s$ and $t$ given a single point obstacle.
We consider a mapping $f : \R \times S^1 \rightarrow S^1 \times \R $ 
taking points in polar coordinates to a transformed plane. 
Given a point $(r, \theta)$ The mapping $f$ is defined as $f(r, \theta) = (\theta, \ln r)$.
\begin{obs}
	The shortest path~$\gamma$ between two points 
	$s$ and $t$ in the transformed plane 
	is the straight-line segment connecting $s$ and $t$.
	Moreover, the length of~$\gamma$ is exactly the Euclidean distance between 
	$s$ and $t$ in the transformed plane.
\end{obs}

To better understand the transformed plane, 
consider a Voronoi cell of a point obstacle in the origin.
Let $y = R$ be  the supporting line of the Voronoi arc 
(which is a straight-line segment).
This line is mapped by $f$ to all points 
$\left(\theta, \ln \left( \frac{R}{\sin \theta} \right) \right)$ which is 
the curve
$$\ln r = \ln R + \ln (\csc \theta). $$


%Let $y = ax + b$ be  the supporting line of the Voronoi arc (which is a straight-line segment).
%This line is mapped by $f$ to all points 
%$\left(\theta, \ln \left( \frac{b}{\sin \theta - a \cos \theta} \right) \right)$.
%If the Voronoi arc lies on the arc $y = y_0$ then it is mapped to the points
%$\left(\theta, \ln \left( \frac{y_0}{\sin \theta} \right) \right)$.
%See Fig.~\ref{fig:transformed_arc}.\oren{add axis to figure}
%\kyle{restrict figure domain to one period of the function}
%
%\begin{figure}[tb]
%  \centering
%   	\includegraphics[height =5.0 cm]{./transformed_1.png}
%	\caption{\sf 	\footnotesize
%				This figure depicts the line 
%				$y = -x + 2$
%				mapped to the transformed plane.}
%  \label{fig:transformed_arc}
%\end{figure}

Next, one may ask how does the boundary of a Voronoi cell map into the transformed plane.
Since we only consider triangulated cells, a triangle~$T$ will consists of two vertical rays starting at $-\infty$ and reaching the curve who is the image of the Voronoi edge.
The rays are at distance at most~$\pi$. 


%Mapping the line using $f$ and taking the lower envelope defined by the set of mapped lines yields the mapped cell.

%
%The Voronoi arcs describing the boundary of a cell are defined by a collection of lines $y= a_i x + b_i$. Mapping each line using $f$ and taking the lower envelope defined by the set of mapped lines yields the mapped cell.
%A possible such cell is depicted in Fig.~\ref{fig:transformed_cell}.\oren{produce better figure}
%\begin{figure}[tb]
%  \centering
%   	\includegraphics[height =5.0 cm]{./transformed_2.jpg}
%	\caption{\sf 	\footnotesize
%				This figure visualizes a possible mapped Voronoi cell.}
%  \label{fig:transformed_cell}
%\end{figure}

\subsection{$O(n)$-approximation algorithm}
\input{easy_approx.tex}

\subsection{Computing the promising nodes of an edge}
Recall that when our Dijkstra-like pass pops a vertex~$u$ from~$\calQ$ such that~$u$ lies in the triangle~$T$ that has an edge~$e$ which had not been sampled yet, 
we wish to compute all the promising nodes lying on~$e$.
Set~$x$ to be the point on~$e$ such that $L^*(u,x)$ is minimal.
Clearly,
if $L^*(u,x) > \OPT$, then no promising nodes lie on~$e$.
Additionally, for all promising nodes~$y$ that lie on~$e$ it holds that $L^*(x,y) < \OPT$
and the shortest path between $x$ and $y$ lies on~$e$ (Lemma~\ref{lem:}\oren{this is the wrong lemma that we need to deal with}.

Thus, one may consider the following approach:
Compute the point~$x$ on~$e$ such that $L^*(u,x)$ is minimal. 
If $L^*(u,x) > \OPT$, then no promising nodes lie on~$e$.
If not, walk on~$e$ in both directions by sampling points at intervals of weighted length $\frac{\eps \OPT}{n}$. 
Clearly, these intervals contain all promising nodes that lie on~$e$ and the number of nodes sampled is $O(\frac{n}{\eps})$.

Thus, we need to explain how to find the closest point~$x$ on~$e$ and how to sample along~$e$ .
% the edge.
%Finding the closest point is not-trivial and we will have to approximate it. We will use the transformed plane described in Section~\ref{sec:transformed}. Sampling along~$e$, however will be done in the original plane.

\paragraph{Approximating the closest point on an edge of~$\calV$ from a point in the same cell}
Recall that the edge~$e$ of a triangle$~T$ can be either an edge added by the triangulation or a Voronoi arc between two obstacles. 
Each triangle~$T$ maps to a pseudo-trapezoid $T'$ bounded by two vertical rays and a convex arc~$e$. 
Finding the point~$v$ for the edges connected to the site is straightforward 
(as they map to vertical rays in the transformed space), 
so we need to describe the procedure for the Voronoi edge
whose equation in the transformed space is 
$\ln r = \ln R + \ln (\csc \theta)$
assuming that the site is origin and the Voronoi edge lies on the horizontal line $y=R$.

Let $u'=(a, \ln b)$ be the image of $u$ in the transformed space. 
Wlog assume that $0 \leq a \leq \pi/2$. 
We are interested in the case when~$u'$ lies inside or on the boundary of $T'$, 
so $u'$ lies below the arc $t$.

Instead of finding the point~$x'$ on~$e$ such that
$\dist{u',x'}$ is minimal, 
we find a point~$v'$ on~$e$ such that~$\dist{u',v'} \leq 2\OPT$. 
This implies that in order to ensure that indeed all promising nodes are within the intervals considered, we need to add~$6\frac{n}{\eps}$ samples along~$e$ 
(instead of at most~$2\frac{n}{\eps}$ samples along~$e$).

Our construction is fairly simple,
First go from $u'$ in the vertical direction by distance at most~$\OPT$ or until~$e$ is intersected .
If~$e$ is intersected, then clearly this intersection point
(i.e., the point $(a,\ln (R/\sin(a)))$
is at distance at most~$\OPT$.
If not, then go in the horizontal direction 
(from the point~$u'' = (a,\ln b + \OPT)$) 
toward the arc by at most~$\OPT$.
If~$e$ is intersected, return that point
(i.e., the point~$(\arcsin{\frac{R}{be^{\OPT}}}, \ln b + \OPT)$). 
Otherwise, one can argue that no point on the arc lies within distance~$\OPT$ from $u'$.\oren{add figure}



\paragraph{Sampling along the Voronoi arcs}
Once the first point~$v$ on the edge~$e$ is sampled, 
we need to sample additional points at intervals of weighted length $O(\frac{\eps \OPT}{n})$ from~$v$.

The edge~$e$ may be
(i)~an edge created by the triangulation or
(ii)~a Voronoi edge.

When~$e$ is an edge of created by the triangulation, 
it is a vertical ray in the transformed plane.
Consider the point~$v$ in the original plane whose image in the transformed plane is~$(\theta_v, \ln r_v)$.
The points at weighted distance $\frac{\eps \OPT}{n}$ from~$v$ are simply~$(\theta_v, \ln r_v \pm \frac{\eps \OPT}{n})$.

When~$e$ is a Voronoi edge, 
we compute the new point directly on the Voronoi.
Following the assumptions of Prop.~\ref{prop:point_point_len}  let~$p_1 = (x_1,y_v)$  and we wish to compute the point~$p_2 = (x_2,y_v)$ such that the path $\gamma^*(p_1, p_2)$ along~$e$ has weighted length $L^*(\gamma^*(p_1, p_2)) = \frac{\eps \OPT}{n}$. 
Using
Eq.~\ref{eq:point_point_len},
$$
\frac{\eps \OPT}{n} 
	= 			
\ln	{\frac	{x_2 + \sqrt{x_2^2 + y_v^2}}
			{x_1 + \sqrt{x_1^2 + y_v^2}}
	}
$$
Using basic algebra we obtain
$
	x_2 = (\kappa^2 - y_v^2) / 2\kappa,
$
for
$
	\kappa = 	\left( x_1 + \sqrt{x_1^2 + y_v^2} \right) 
					\cdot
				e^{\eps \OPT / n}
$.

%
%
%
%\subsection{Approximating the closest point on an edge of~$\calV$ from a point in the same  cell}
%\label{subsec:apx_closest_point}
%Recall that while computing the shortest path from~$s$ towards~$t$,
%we need to approximate the closest point on an edge of~$\calV$ from a point in the same Voronoi cell.
%Specifically, we consider a vertex~$u$ lying on the boundary of a triangle~$T$.
%We wish to compute a point~$v$ on~$e$ 
%such that Eq.~\ref{eq:almost-closest} holds (namely that~$v$ is no more than twice the distance from~$u$ than the closest point on the boundary).
%
%Each triangle~$T$ maps to a pseudo-trapezoid $T'$ bounded by two vertical rays and a convex arc~$e$. 
%Finding the point~$v$ for the edges connected to the site is straightforward 
%(as they map to vertical rays in the transformed space), 
%so we need to describe the procedure for the Voronoi edge
%whose equation in the transformed space is 
%$\ln r = \ln R + \ln (\csc \theta)$
%assuming that the site is origin and the Voronoi edge lies on the horizontal line $y=R$.
%
%Let $u'=(a, \ln b)$ be the image of $u$ in the transformed space. 
%Wlog assume that $0 \leq a \leq \pi/2$. 
%We are interested in the case when~$u'$ lies inside or on the boundary of $T'$, 
%so $u'$ lies below the arc $e$.
%
%The slope of the tangent of $e$ at $\theta$ is $-\cot\theta$. 
%Let $\xi$ be the point on $e$ at $\theta=\pi/4$; 
%the slope of~$e$ at $\xi$ is $-1$. 
%Let 
%  $\ell_x$ be the ray emanating from $\xi$ in $-x$ direction and 
%  $\ell_y$ the ray emanating from $\xi$ in $-y$ direction.
%(i)~If $u'$ lies above the line $\ell_x$, 
%then set $v$ to be the intersection point of $e$ with the horizontal line passing through $u'$
%%(i.e., the point $(\frac{1}{\sin (b/R)}, b)$ 
%(see Fig.~\ref{fig:closest_points_1}).
%(ii)~If $u'$ lies to the right of $\ell_y$
%then set $v$ to be the intersection point of $e$ with the vertical line passing through $u'$ 
%%(i.e., the point $(a,\ln (R/\sin(a)))$
%(see Fig.~\ref{fig:closest_points_2}).
%(iii)~Otherwise, take~$v$ to be the intersection point if~$e$ with the line with slope 1 passing through~$u'$. 
%(see Fig.~\ref{fig:closest_points_3}\oren{change v to be v' as v is in the original plane}).
%
%
%\begin{figure*}[tbh]
%  \centering
%  \subfloat
%   [\sf Case~(i)]
%   { 
%   	\includegraphics[width =5 cm]{closest_points_1.pdf}
%   	\label{fig:closest_points_1}
%   }
%   \hspace{3mm}
%  \subfloat
%   [\sf Case~(ii)]
%   {
%   	\includegraphics[width =5 cm]{closest_points_2.pdf}
%   	\label{fig:closest_points_2}
%   }
%   \hspace{3mm}
%  \subfloat
%   [\sf Case~(iii)]
%   {
%   	\includegraphics[width =5 cm]{closest_points_3.pdf}
%   	\label{fig:closest_points_3}
%   }
%  \caption{\sf 	Different cases considered for approximating the 
%  				closest point on an edge~$e$ of~$\calV$ 
%  				from a point in the same cell.
%  				The image~$e$ of~$e$ is depicted in blue and 
%  				the tangent at $\pi/4$ is depicted in orange.
%  }
%  \label{fig:cont}
%\end{figure*}
%
%
%
%We still need to show that for each case indeed
%Eq.~\ref{eq:almost-closest} holds
%and how to construct (or approximate) the 
%pre-image of each curve in the original space. 
%
%We show that Eq.~\ref{eq:almost-closest} holds for the case~(i), other cases follow similar lines of reasoning.
%Set~$\tilde{x'}$ to be the closest point to $u$ along the boundary and denote by $\theta_v$ the angle attained at point~$v$. 
%We first note that~$\tilde{x'}$ cannot be between~$v$ and~$\xi$. 
%Now, as the slope is monotonically decreasing,	 all points on the boundary with $\theta \leq \theta_v$ (and~$\tilde{x'}$ in particular) lie above the line with slope~$-1$ passing through~$v$.
%Denote this line by $\ell_v$ and notice that the distance between $u'$ and $\ell_v$ gives a lower bound on the distance between~$u'$ and~$\tilde{x'}$).
%This distance is $\frac{\sqrt2}{2} L^*(u', v')$ which concludes the argument.
%See fig.~\ref{fig:closest_proof}.
%
%\begin{figure}[tb]
%  \centering
%   	\includegraphics[height =5.0 cm]{./closest_proof.pdf}
%	\caption{\sf 	\footnotesize
%				Proof of Eq.~\ref{eq:almost-closest} for case~(i) of the construction in Section~\ref{subsec:apx_closest_point}.
%				Blue curve depicts the boundary of the Voronoi cell in the transformed plane, gold line depicts the line of slope~$-1$ passing through the constructed point~$v$. 
%			}
%  \label{fig:closest_proof}
%\end{figure}
%
%
%%It can be shown that ||u'v|| \le 2\min_{x\in g} ||u'x||.
%%[I'll try to send you a figure, which I hope will help you understand what I am talking about.]
%%
%%Horizontal and vertical lines in the transformed space have nice pre-image in the original space. 
%%The former is a circular arc centered at origin, 
%%and the latter is a radial line passing through the origin. 
%%I don't know if the line with the slope 1 also has a nice pre-image. If not we can approximate it.
%
%
%
%
%\subsection{Sampling along the Voronoi arcs}
%Recall that our algorithm samples at most $O(\frac{n}{\eps})$ points on each arc of our triangulation.
%The points are sampled at intervals of weighted length $O(\frac{\eps \OPT}{n})$.
%More specifically, once we find the first point~$v$ on an edge~$e$, 
%we need to sample points at distance at most $2\OPT$\oren{this constant may should be worked out, it could be slightly larger since we don't get the closest point to $u$... } in each direction along~$e$. 
%
%
%The edge~$e$ may be
%(i)~an edge created by the triangulation or
%(ii)~a Voronoi edge.
%
%When~$e$ is an edge of created by the triangulation, 
%it is a vertical ray in the transformed plane.
%Consider the point~$p$ in the original plane whose image in the transformed plane is~$(\theta_p, \ln r_p)$.
%The points at weighted distance $\frac{\eps \OPT}{n}$ it are simply~$(\theta_p, \ln r_p \pm \frac{\eps \OPT}{n})$.
%
%When~$e$ is a Voronoi edge, 
%we compute the new point directly on the Voronoi.
%Following the assumptions of Prop.~\ref{prop:point_point_len}  let~$p_1 = (x_1,0)$  and we wish to compute the point~$p_2 = (x_2,0)$ such that the path $\gamma^*(p_1, p_2)$ along~$e$ has weighted length $L^*(\gamma^*(p_1, p_2)) = \frac{\eps \OPT}{n}$. 
%Using
%Eq.~\ref{eq:point_point_len},
%$$
%\frac{\eps \OPT}{n} 
%	= 			
%\ln	{\frac	{x2 + \sqrt{x_2^2 + y_v^2}}
%			{x1 + \sqrt{x_1^2 + y_v^2}}
%	}
%$$
%Using basic algebra we obtain
%$
%	x_2 = (\kappa^2 - y_v^2) / 2\kappa,
%$
%for
%$
%	\kappa = 	\left( x_1 + \sqrt{x_1^2 + y_v^2} \right) 
%					\cdot
%				e^{\eps \OPT / n}
%$.

\subsection{Reducing the number of edges}
Recall, that we sample $O(\frac{n}{\varepsilon})$ points on each edge.
Thus, the number of edges in a triangle could be as large as $O(\frac{n^2}{\varepsilon^2})$.
To reduce the number of edges considered we build a spanner over the vertices in each triangle.
Recall that in the transformed plane, the weighted distance is transformed to Euclidean distances.
Thus, we construct the $\Theta$-graph (see~\cite{ASY09, C87}) over these samples.
If we use the construction by Clarkson~\cite{C87}, this takes~$O\left(\frac{n}{\eps^2} \log \frac{n}{\eps} \right)$ time and the number of edges in each cell is~$\left(\frac{n}{\eps^2}\right)$. 

\subsection{Analysis}
\paragraph{Size of graph}
Recall that $n$ denotes the number of obstacles.
The Voronoi diagram$~\calV$ contains a linear number of vertices  and edges.
%$2n - 5$ Voronoi vertices 
%and
%$3n - 6$ Voronoi edges. 
We triangulate this in order to have cells of constant complexity but remain with a linear number of edges in our triangulation.
On each edge we sample $O(\frac{n}{\eps})$, thus we have a total of $V = O(\frac{n^2}{\eps})$ vertices.
As we construct a spanner in each cell, we have $E = O(\frac{n^2}{\eps^2})$ edges in total.

\paragraph{Running time}
Building the  Voronoi diagram$~\calV$ requires $O(n \log n)$ time. 
Building the spanner in each triangle takes $O\left(\frac{n^2}{\eps^2} \log \frac{n}{\eps} \right)$ time. 
Finally, we run our Dijkstra-like search which takes $O(E + N \log N)$ time.
Thus, the total running time of one iteration of our algorithm is dominated by the spanner construction and is
$$
O\left(\frac{n^2}{\eps^2} \log \frac{n}{\eps} \right)$$.
Finally, we do this  $O(\log n)$ iterations such that the final running time is
$$
O\left(\frac{n^2}{\eps^2} \log \frac{n}{\eps} \log n \right)$$.


\paragraph{Approximation factor}
Following similar arguments as in~\cite{WBH08} our algorithm returns a path whose cost has a multiplicative  of $1 + \eps$ and an additive factor of $\eps$. 


%Our algorithm computes an $O(n)$-approximation on $d^*$ and then does a binary search for $d^*$,
%applying each guess to the following procedure.
%We assume from here on that the algorithm knows $d^*$.
%
%Let $\lambda$ be Voronoi arc, 
%defined by two point obstacles $o_1, o_2$.
%Assume that $o_1, o_2$ are the only obstacles.
%For every point $x$ lying on $\lambda$, 
%denote by $L^*(s,x)$ and $L^*(t,x)$ the cost of the shortest path connecting $s$ and $t$ to $x$, respectively.
%If $L^*(s,x) +  L^*(x,t)> d^*$ 
%when only taking $o_1$ and $o_2$ into account
%then the optimal path between $s$ and $t$ cannot pass through $x$.
%This is true because travel costs only increase when additional obstacles are added.
%We refer to all points~$x$ lying on a Voronoi arc~$\lambda$ such that 
%$L^*(s,x) +  L^*(x,t) \leq d^*$ as $(s,t)$-\emph{promising points}.
%
%\begin{obs}
%\label{obs:length}
%For any two  $(s,t)$-promising points $x_1, x_2$ lying on the same Voronoi arc~$\lambda$, 
%denote by $\lambda(x_1, x_2)$ the piece of $\lambda$ connecting $x_1$ and $x_2$ and recall that this is the optimal path between $x_1$ and $x_2$.\oren{This statement is NOT true by Kyle's example. We should address this point.}
%If all points on $\lambda(x_1, x_2)$ are promising then by the triangle inequality 
%$L^*(\lambda(x_1, x_2)) \leq L^*(x_1,s) +  L^*(s,x_2) \leq 2d^*$.
%\end{obs}
%
%Let $\calV_{d^*}(s,t)$ denote all the $(s,t)$-promising points lying on the Voronoi Diagram~$\calV$ of the obstacle points. 
%\begin{lem}
%	The weighted length of $\calV_{d^*}(s,t)$, 
%	denoted by $\Lambda_{d^*}(s,t)$ is bounded by
%	$$
%		\Lambda_{d^*}(s,t) \leq 12n \cdot d^*
%	$$
%\end{lem}
%
%\begin{proof}
%Recall that using Euler's formula the number of edges in the Voronoi diagram of a set of $n$ points is bounded by $3n-6$.
%By Lemma~\ref{lem:intervals} each Voronoi edge can contribute at most two different continuous arcs to $\calV_{d^*}(s,t)$.
%By Obs.~\ref{obs:length} the length of each arc is at most $d^*$ thus
%$\Lambda_{d^*}(s,t) \leq (3n-6) \cdot 2 \cdot 2 \cdot d^* \leq 12n \cdot d^*$.
%\end{proof}
%
%We can now consider a similar approach to the one taken by Wein \etal~\cite{WBH08} for choosing portals.
%Recall that Wein \etal subdivide all Voronoi arcs into intervals such that the length of an interval $I$ is $\cl(I) \eps / (24 n)$. 
%This, in turn, implied that they consider $(24 \Lambda n )/ \eps$ intervals (where $\Lambda$ denotes the weighted length of $\calV$).
%We do the same but restrict ourselves to 
%$\calV_{d^*}(s,t)$.
%Hence we only have 
%$\frac{24 \Lambda_{d^*}(s,t) n }{\eps} 
%	\leq 
%\frac{252 n^2  \cdot d^*}{\eps} $ intervals.


==> point_obs_sp.tex <==
\section{Shortest paths between in a Voronoi cell of point obstacles}
Cor.~8 in Wein \etal states that the optimal path between two points~$s$ and~$t$ on a Voronoi arc~$\lambda$ of any kind is the piece of ~$\lambda$  between~$s$ and~$t$. This does not hold when only point obstacles are considered.
As a counterexample, suppose we only have obstacles at 
$(0,-1)$ and $(0,1)$
and we want to travel from $(-x, 0)$ to $(x, 0)$ 
which both lie on the one Voronoi arc between the obstacles. 
Suppose $x \gg 1$. 
Travelling along the arc has cost roughly equal to $2 \ln x$. 
A better solution would be to follow a nearly circular arc above the
obstacle at $(0,1)$ for a cost roughly equal to~$\pi$.
See Fig.~\ref{fig:sp} for a visualization.

\begin{figure*}[tbh]
  \centering
  \subfloat
   [\sf Workspace]
   { 
   	\includegraphics[height =3.5 cm]{sp.pdf}
   	\label{fig:sp_workspace}
   }
   \hspace{3mm}
  \subfloat
   [\sf Transformed plane]
   {
   	\includegraphics[height =3.5 cm]{sp_transformed.pdf}
   	\label{fig:sp_transformed}
   }
  \caption{\sf 	Path between two points~$s$  and~$t$ on the 
  				boundary of a Voronoi cell in the workspace~(a) and in the 
  				transformed plane (b).
  				The path along the boundary of the cell is depicted in red 
  				while the shortest weighted path is depicted in 
  				green.}
  \label{fig:sp}
\end{figure*}

Given a point $s$ in a Voronoi cell, 
one may wish to find all points that are of distance at most $r$ from $s$ on a Voronoi arc $\lambda$.
The transformed cell allows us to easily  argue that all such points do not necessarily lie on a continuous piece of $\lambda$.
This is because the mapping of $\lambda$ to the transformed cell is not continuous.
See Fig.~\ref{fig:cont} for a visualization.


\begin{figure*}[tbh]
  \centering
  \subfloat
   [\sf Workspace]
   { 
   	\includegraphics[height =3 cm]{cont.pdf}
   	\label{fig:cont_workspace}
   }
   \hspace{3mm}
  \subfloat
   [\sf Transformed plane]
   {
   	\includegraphics[height =3 cm]{cont_transformed.pdf}
   	\label{fig:sp_transformed}
   }
  \caption{\sf 	Visualization of all points of distance $r$ away from a 
  				point $s$ on the boundary of a a Voronoi cell in the 
  				workspace~(a) and 
  				in the transformed plane (b).}
  \label{fig:cont}
\end{figure*}


This leads us to the following observation
\begin{obs}
\label{obs:intervals}
	Let~$\lambda$ be a Voronoi arc in a Voronoi cell $c$ and
	$p$ be a point in $c$.
	The set of points that are of distance exactly~$r$ from~$p$ 
	that lie on~$\lambda$ lie on at most two different continuous  
	pieces of $\lambda$.
\end{obs}



==> spanner.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Approximating the boundary of a Voronoi cell of a point}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we show how to approximate the boundary of a Voronoi cell of a point obstacle into a convex obstacle.
The construction is fairly simple. 
We are given two points~$p_1,p_2$ on a Voronoi edge $e$ whose weighted length is $d$ and we want to approximate the portion of the curve~$g$ connecting the points in the transformed plane such that:
(i)~the length of this polyline is exactly $d$,
(ii)~for every point~$q$, the straight-line segment (in the transformed plane)~$\overline{p_i q}$ intersects the polyline iff it intersects~$g$.

Let $p_1', p_2'$ denote the points~$p_1,p_2$ in the transformed plane. 
Let $t_1, t_2$ denote the tangents at $p_1', p_2'$,
$q_1', q_2'$ the points on $t_1, t_2$ of (Euclidean) length 
$\alpha \cdot d$ in the direction of $p_2', p_1'$, respectively.
The polyline is defined as $(p_1', q_1', q_2', p_2')$.

\paragraph{Equation of the tangent}
Let $\ln r = m_i \theta + n_i$ be the equation of the tangent $t_i$ for point
$p_i' = (\theta_{p_i'}, \ln \frac{R}{sin\theta_{p_i'}})$.
Clearly,
$$
	m_i = - \cot \theta_{p_i'}
	\text{ \hspace{5mm} and \hspace{5mm} }
	n_i = \ln {\frac{R}{sin \theta_{p_i'}}} + \theta_{p_i'} \cdot \cot \theta_{p_i'}.
$$

\paragraph{Coordinates of the points on tangents}
Recall that we are looking for the point at distance
$\alpha \cdot d$ from $p_i$ on $t_i$.
Thus,
$$
	\dist{q_i', p_i'}^2 
	= 
	(\theta_{q_i'} - \theta_{p_i'})^2
	+
	(\ln r_{q_i'} - \ln r_{p_i'})^2	
$$
where,
$$
	\ln r_{p_i'} = \ln \frac{R}{sin\theta_{p_i'}}
	\text{ \hspace{5mm} and \hspace{5mm} }
	\ln r_{q_i'} =  m_i \theta_{q_i'} + n_i.
$$
Hence,
$$
	(\alpha \cdot d)^2 
	= 
	(\theta_{q_i'} - \theta_{p_i'})^2
	+
	( m_i \theta_{q_i'} + n_i -\ln \frac{R}{sin\theta_{p_i'}})^2	
$$
Substituting for $m_i, n_i$,
$$
	(\alpha \cdot d)^2 
	= 
	(\theta_{q_i'} - \theta_{p_i'})^2
	+
	( - \cot \theta_{p_i'} \theta_{q_i'} + \ln {\frac{R}{sin \theta_{p_i'}}} + \theta_{p_i'} \cdot \cot \theta_{p_i'} -\ln \frac{R}{sin\theta_{p_i'}})^2	
$$
Which, in turn, yields,
$$
	(\alpha \cdot d)^2 
	= 
	(\theta_{q_i'} - \theta_{p_i'})^2
	+
	(-\cot \theta_{p_i'} 
		\cdot 
	(\theta_{q_i'} - \theta_{p_i'}))^2	
$$
simplifying this gives,
$$
	(\alpha \cdot d)^2 
	= 
	(\theta_{q_i'} - \theta_{p_i'})^2
	\cdot
	(1 +\cot^2 \theta_{p_i'})
$$
which gives
$$
	\theta_{q_i'} 
	= 
	\pm \frac{\alpha \cdot d}{\sqrt{1 + cot^2 \theta_{p_i'}}}
	+ \theta_{p_i'}
$$
Using the identity 
$\sin \theta = \pm \frac{1}{\sqrt{1 + \cot \theta}}$ 
we obtain:
\begin{equation}
	\theta_{q_i'} 
	= 
	\frac{\alpha \cdot d}{\sin \theta_{p_i'}}
	+ \theta_{p_i'}
\end{equation}
Recall that $\ln r_{q_i'} =  m_i \theta_{q_i'} + n_i$.
Thus,
$$
	\ln r_{q_i'} =  
	- \cot \theta_{p_i'} \cdot (\frac{\alpha \cdot d}{\sin \theta_{p_i'}}
	+ \theta_{p_i'}) + \ln {\frac{R}{sin \theta_{p_i'}}} + \theta_{p_i'} \cdot \cot \theta_{p_i'}
$$
which can be simplified to 
\begin{equation}
	\ln r_{q_i'} 
	=  - \frac{\cot \theta_{p_i'}}{\sin \theta_{p_i'}} 
		\cdot (\alpha \cdot d)
		+
		\ln {\frac{R}{sin \theta_{p_i'}}} 
\end{equation}

\paragraph{the points $p_1, p_2$}
Recall that the points $p_1, p_2$ are distance $d$ apart.
If the obstacle is at the origin and
$p_1 = (x_1, R)$ then
$p_2 = (\frac{\kappa^2 - R^2}{2\kappa})$ where
$\kappa = (x_1 + \sqrt{x_1^2 + R^2})\cdot e^d$.
Note that:
$$
	\sin \theta_{p_i} = \frac{R}{r_i}
	\text{ \hspace{5mm} and \hspace{5mm} }
	\cos \theta_{p_i} = \frac{x_i}{r_i}
	\text{ \hspace{5mm} and \hspace{5mm} }
	\cot \theta_{p_i} = \frac{x_i}{R}
$$
where, $r_i = \sqrt{x_i^2 + R^2}$.

Now, for $p_1$:
$$
	\sin \theta_{p_1} = \frac{R}{\sqrt{x_1^2 + R^2}}
	\text{ \hspace{5mm} and \hspace{5mm} }
	\cos \theta_{p_1} = \frac{x_1}{\sqrt{x_1^2 + R^2}}
	\text{ \hspace{5mm} and \hspace{5mm} }
	\cot \theta_{p_1} = \frac{x_1}{R}
$$


==> visibility.tex <==
\section{Visibility}

Let~$T$ be a cell of~$\dvd$ incident to polygon segment~$o$.
We say two points~$p$ and~$q$ in~$T$ are \emph{visible} to one another if their
minimal-cost path relative to~$\calO$ is the same as their minimal-cost path relative to~$o$ only.

The following lemma should be copied over to the PTAS section.
\begin{lem}
\label{lem:visibility}
Let~$T$ be a cell of~$\dvd$ incident to polygon segment~$o$.
Let~$p$ be a point on~$T$'s boundary, and let~$e_0 \neq o$ be an edge of~$T$ not containing~$p$.
Let~$Q_p$ be the set of points~$q$ on~$e_0$ visible to~$p$.
If~$Q_p$ is non-empty, then it is connected and has one boundary at an endpoint of~$e_0$.
\end{lem}
\begin{proof}
Let~$e$ be the standard arc of~$T$.
Let~$\alpha$ and~$\beta$ be the shorter and longer vertical arcs of~$T$ respectively, and let~$u$
and~$v$ be the vertices connecting~$\alpha$ and~$\beta$ to~$e$ respectively.
We consider two main cases.\\

\textbf{Case 1)} Suppose~$o$ is a polygon vertex.
Without loss of generality,~$o$ lies at the origin, edge~$\alpha$ intersects the line~$y = 0$ at
the origin with angle~$\theta_{\alpha}$,
edge~$\beta$ intersects the line~$y = 0$ at the origin with angle~$\theta_{\beta}$,
and~$\theta_{\beta} > \theta_{\alpha} \geq 0$.
Let~$q \in Q_p$.
If~$q$ does not exist, then there is nothing to prove.
Otherwise, let~$\gamma$ be the minimal-cost path from~$p$ to~$q$.
Eq.~\ref{eq:length_point} describes the cost of~$\gamma$.
We consider a mapping $f : \R \times S^1 \rightarrow S^1 \times \R $ 
taking points in polar coordinates to a transformed plane. 
Given a point $(r, \theta)$, the mapping $f$ is defined as $f(r, \theta) = (\theta, \ln r)$.
Given a path~$\gamma'$, we abuse notation and let~$f(\gamma')$ equal the application of~$f$ to
each point of~$\gamma'$.
Path~$\gamma$ becomes a line segment connecting $p$ and $q$ in the transformed plane.
Both~$\alpha$ and~$\beta$ become vertical rays in the transformed plane going to~$-\infty$.
Further, it is straightforward to show that~$e$ becomes a convex curve in the transformed plane
when restricted to values of~$\theta$ such that~$\theta_{\alpha} \leq \theta \leq \theta_{\beta}$.
Two points~$p'$ and~$q'$ in~$T$ are visible if and only if the line segment between~$f(p')$
and~$f(q')$ does not cross any component of~$T$ in the transformed plane.

Suppose~$p$ lies on~$\alpha$.
Point~$u$ is clearly visible to~$p$.
Let~$\gamma_{u,p}$ be the line segment from~$p$ to~$u$.
Transformed plane segment~$f(\gamma_{u,p})$ is supported by a line~$\ell$ with infinite slope;
line~$\ell$ contains the point~$(\theta, \infty)$ for every~$\theta \geq \theta_{\alpha}$.
Imagine decreasing the slope of~$\ell$ continuously.
The first intersection of~$\ell$ with~$f(e)$ moves farther to the right as you do so.
Each of these first intersections are visible to~$p$.
Line~$\ell$ eventually goes tangent to~$f(e)$ at~$(\theta^*,\ln r^*)$, and never intersects it
again after that point.
Let~$\ell^*$ be this tangent line.
Line~$\ell^*$ is the first line to intersect~$\beta$ without first crossing~$f(e)$.
If~$e_0 = e$, then~$Q_p$ consists of all points~$q$ such that~$f(q)$ lies on~$f(e)$
between~$f(u)$ and~$(\theta^*, \ln r^*)$.
If~$e_0 = \beta$, then~$Q_p$ consists of all points~$q$ such that~$f(q)$ lies on~$\beta$ below the
intersection of~$f(\beta)$ and~$\ell^*$.
A similar argument holds if~$p$ lies on~$\beta$.

Finally, suppose~$p$ lies on~$e$ and~$e_0 = \alpha$.
Let~$\ell^*$ be the line tangent to~$f(e)$ at~$f(p)$.
Line~$\ell^*$ intersects~$f(\alpha)$ at~$f(w)$.
Lines to higher points on~$f(\alpha)$ cross~$f(e)$, so~$w$ is the highest clearance point
on~$\alpha$ visible to~$p$.
All lower points on~$f(\alpha)$ are visible, though.
Therefore,~$Q_p$ consists of all points~$q$ on~$\alpha$ of clearance at most~$\cl(w')$.
A similar argument holds if~$p$ lies on~$e$ and~$e_0 = \beta$.\\

\textbf{Case 2)} Suppose~$o$ is a polygon edge.
Without loss of generality, $o$ lies on the line~$y = 0$, the edge~$\alpha$ lies on the line~$x =
x_{\alpha}$, the edge~$\beta$ lies on the line~$x = x_{\beta}$, and~$x_{\beta} > x_{\alpha} \geq
0$.
There is no notion of the transformed plane for polygon edge~$o$, but we are still able to use
similar arguments to those given in Case 1.
Two points~$p'$ and~$q'$ in~$T$ are visible if the circular arc containing~$p'$ and~$q'$
centered on~$o$ does not cross~$e$.

Suppose~$p$ lies on~$\alpha$.
Point~$u$ is clearly visible to~$p$.
The circle~$C$ containing the minimal-cost path from~$u$ to~$p$ has a center at~$(\infty, 0)$, and
its upper half contains the point~$(x, \infty)$ for every~$x > 0$.
Imagine continuously moving the center of~$C$ to the left.
Edge~$e$ is a convex curve, and the upper half of~$C$ is a concave curve; they intersect at at
most~$2$ points at any moment during this procedure.
Fix an~$x > 0$.
As the center of~$C$ moves left, the point~$(x,y)$ in the upper half of the circle continuously
moves downward until it reaches~$(x,0)$ and disappears;
indeed, the bisector of line segment~$p(x,y)$ must continue intersecting the center~$C$ as the
center moves left.
Therefore,~$C$ and~$e$ eventually stop crossing; this event even occurs when~$C$ and~$e$ go
tangent at point~$w^* = (x^*, y^*)$.
Let~$C^*$ be this circle tangent to~$e$.

Circle $C$ initially lies above~$e$ at each~$x$-coordinate, but eventually it lies below~$e$ at
each ~$x$-coordinate.
Also, the second crossing of~$C$ and~$e$ can never occurs to the left of~$w^*$ during the
procedure.
We conclude that each point~$(x,y)$ on~$e$ between~$u$ and~$w^*$ must be visible from~$p$.
If~$e_0 = e$, then these points are precisely~$Q_p$.

Now, assume some point on~$\beta$ is visible to~$p$.
The moment when~$C$ goes tangent to~$e$ at~$w^*$ is also the first moment when~$C$ does not
cross~$e$ before reaching~$\beta$.
As the center of~$C$ continues moving left, the intersection of~$C$ and~$\beta$ continuously moves
downward.
If~$e_0 = \beta$ and~$Q_p$ is non-empty, we have~$Q_p$ consisting of all points on~$\beta$
between~$o$ and the intersection of~$C^*$ and~$\beta$.
A similar set of arguments hold if~$p$ lies on~$\beta$.

Finally, suppose~$p$ lies on~$e$ and~$e_0 = \alpha$.
Let~$C^*$ be the circle centered on~$o$ which lies tangent to~$e$ at~$p$.
Circle~$C^*$ contains a point~$q^*$ on~$\alpha$ visible to~$p$.
If we initially take~$C = C^*$ and move the center of~$C$ to the left, then the arc between~$p$
and~$\alpha$ along~$C$ moves above~$e$ and must cross again closer to~$\alpha$.
However, if we move the center of~$C$ to the right, then the arc between~$p$ and~$\alpha$ stays
below~$e$.
In addition, the intersection of~$C$ and~$\alpha$ moves downward.
Therefore~$Q_p$ consists of all points~$q$ such that~$q$ lies on~$\beta$ below~$q^*$.
A similar argument holds if~$p$ lies on~$e$ and~$e_0 = \beta$.
\end{proof}

